On the convergence of adaptive first order methods: proximal gradient and alternating minimization algorithms

Building upon recent works on linesearch-free adaptive proximal gradient methods, this paper proposes adaPG$^{q,r}$, a framework that unifies and extends existing results by providing larger stepsize policies and improved lower bounds. Different choices of the parameters $q$ and $r$ are discussed and the efficacy of the resulting methods is demonstrated through numerical simulations. In an attempt to better understand the underlying theory, its convergence is established in a more general setting that allows for time-varying parameters. Finally, an adaptive alternating minimization algorithm is presented by exploring the dual setting. This algorithm not only incorporates additional adaptivity, but also expands its applicability beyond standard strongly convex settings.

==> TeX/Preamble.tex <==
%!TEX root = ../adaAMA.tex
\makeatletter
	\ifarticleclass\arxivtrue\fi

%% Packages ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

	\PassOptionsToPackage{noend}{algpseudocode}
	\PassOptionsToPackage{breakspaces}{clevethm}

	\usepackage{bbm}
	\usepackage{colortbl}
	\usepackage{mathrsfs}

	\ifarticleclass
		\usepackage[%
			arxiv,
% 			noqed,
			alglinenumber,
			eqreset=section,
			thmreset=section,
		]{myPreamble}
	\else
		\usepackage{thm-restate}
		\usepackage{times}
		\let\set\undefined
		\newcommand{\theoremstyle}[1]{}
		\usepackage{pgffor}
		\foreach \x/\X in {ass/assumption, cor/corollary, defin/definition, es/example, fact/fact, lem/lemma, prop/proposition, rem/remark, thm/theorem} {
			\expandafter\expandafter\expandafter\global\expandafter\let\csname\X\endcsname\relax
			\expandafter\expandafter\expandafter\global\expandafter\let\csname c@\X\endcsname\relax
		}%

		\usepackage[%
			noqed,
			alglinenumber,
			eqreset=section,
			thmreset=section,
			customsettings=false,
			verbose=false,
			noload={amsthm,caption,subcaption},%
		]{myPreamble}
	\fi



%% Frontmatter ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

	\ifarticleclass\else
		\renewcommand{\TheAddressKU}{%
			Department of Electrical Engineering (ESAT-STADIUS)\\
			KU Leuven, Kasteelpark Arenberg 10, 3001 Leuven, Belgium%
		}
		\renewcommand{\TheAddressKUJ}{%
			Faculty of Information Science and Electrical Engineering (ISEE)\\
			Kyushu University, 744 Motooka, Nishi-ku 819-0395, Fukuoka, Japan%
		}
	\fi

	\ifarticleclass
		\newcommand{\AND}{\ \(\cdot\)\ }
	\else
		\newcommand{\AND}{,\ }
	\fi



%% Typesetting ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

	\urlstyle{sf}
	\frenchspacing
	\def\myampersand{&}
	\newcommand{\arXivLink}[1]{\href{https://arxiv.org/abs/#1}{arXiv:#1}}
	\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
	\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}



%% Theorems ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

	\counterwithin{assumption}{section}
% 	\renewcommand{\theassumption}{\arabic{assumption}}

	\ifarticleclass
		\newcommand{\noqed}{}

	\else

		\setlistoptions{itemsep=2pt, labelsep=3pt, leftmargin=*, align=right, before={\noindent\hspace*{0pt}}}
		\setlistoptions[proofitemize]{itemsep=2pt, labelsep=3pt, leftmargin=*, align=right, before={\noindent\hspace*{0pt}}}

		\setlistlabel[enumerate,1]{\textit{(\roman*)}}
		\setlistlabel[enumerateq,1]{\textit{(\alph*)}}
		\setlistlabel[enumerator,1]{\textit{(\Alph*)}}
		\setlistlabel[enumeratass,1]{A\oldstylenums{\arabic*}}
		\setlistlabel[enumeratprop,1]{P\oldstylenums{\arabic*}}
		\setlist[proofitemize,1]{leftmargin=0pt,label={},labelindent=\parindent,itemsep=\baselineskip}
		\setlistlabel[proofitemize,1]{\labelitemi}
		\setlistlabel[proofitemize,2]{\labelitemii}

		\setlistlabel[2]{\oldstylenums{\arabic*}.}

		\apptocmd\remark{\normalfont}{}{}
		\crefname{definition}{Definition}{Definitions}
		\crefname{lemma}{Lemma}{Lemmas}
		\crefname{remark}{Remark}{Remarks}

		\newcommand{\pushQED}[1]{\qedhere}
		\newcommand{\popQED}{\noqed}
		\newcommand{\qedhere}{\jmlrQED}
		\newcommand{\noqed}{\let\jmlrQED\relax}

		\pretocmd\endappendixproof{\qedhere}{}{}

	\fi

	\newlist{claims}{enumerate}{1}
	\setlist[claims,1]{
		label={\it Claim \oldstylenums{\arabic*}:},
		ref={\oldstylenums{\arabic*}},
		partopsep=0pt,
		parsep=0pt,
		itemsep=3pt,
		wide,
		labelindent=0pt,
	}
	\newlist{claims*}{enumerate}{1}
	\setlist[claims*,1]{
		label={\it Contradiction claim \oldstylenums{\arabic*}$^*$:},
		ref={\oldstylenums{\arabic*}$^*$},
		partopsep=0pt,
		parsep=0pt,
		itemsep=3pt,
		wide,
		labelindent=0pt,
	}
	\Crefname{claimsi}{Claim}{Claims}



%% References ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

	\Crefname{figure}{Figure}{Figures}
	\newcommand{\secref}{\@ifstar\@@secref\@secref}
	\newcommand{\@secref}[1]{\hyperref[#1]{\S}\ref{#1}}
	\newcommand{\@@secref}[1]{\S\ref*{#1}}



%% Algorithms ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

	\renewcommand{\algorithmiccomment}[1]{\hfill{\color{gray}\sf\small//\ (#1)}}
	\crefname{ALG@line}{step}{steps}
	\numberwithin{algorithm}{section}

	\newcommand{\algnamefont}{\sffamily}

	\newcommand{\adaPG}{{\algnamefont adaPG}}%
	\newcommand{\refadaPG}{\hyperref[alg:adaPG]{{\algnamefont AdaPG}\(^{\rp,r}\)}}
	\newcommand{\refadaAMA}{\hyperref[alg:adaAMA]{{\algnamefont AdaAMA}\(^{\rp,r}\)}}


	\NewEnviron{myalg}[2][]{%
		\par\addvspace{\baselineskip}
		\phantomsection
		\par\noindent\hspace*{0pt}\hfill
		\ifstrempty{#1}{}{%
			\label{#1}%
		}%
		\fbox{%
			\begin{minipage}{0.9\linewidth}
				\textbf{#2}\quad\small
				\BODY
			\end{minipage}
		}%
		\hfill\hspace*{0pt}
		\par\noindent
		\vspace{.25\baselineskip}%
		\par
	}


%% Math ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

	\DeclareMathOperator{\m}{m}
	\def\innprod{\@ifstar\@innprod\@@innprod}

	\newcommand{\rp}{q}
	\renewcommand{\pi}{\rp}


	\let\textl\l
	\let\textL\L
	\DeclareRobustCommand{\l}{\ifmmode\ell\else\textl\fi}
	\DeclareRobustCommand{\L}{\ifmmode L\else\textL\fi}
	\newcommand{\M}{L}
	\newcommand{\U}{\mathcal U}
	\newcommand{\V}{\mathcal V}

	\def\innprod{\@ifstar\@innprod\@@innprod}

	\newcommand{\Lagr}{\mathscr{L}}

	\newcommand{\lk}{\@ifstar{\l_{k+1}}{\l_k}}

	\let\oldalpha\alpha\renewcommand{\alpha}{\asdasdfasddff}
	\let\oldbeta\beta\renewcommand{\beta}{\asdasdfasddff}
	\let\oldnu\nu\renewcommand{\nu}{\text{\huge\red$\oldnu$}}


	\newcommand{\alphk}{\@ifstar{\alpha_{k+1}}{\alpha_k}}%
	\newcommand{\betk}{\@ifstar{\beta_{k+1}}{\beta_k}}%
	\newcommand{\delk}{\@ifstar{\delta_{k+1}}{\delta_k}}%
	\newcommand{\thetk}{\@ifstar{\vartheta_{k+1}}{\vartheta_k}}%
	\newcommand{\gamk}{\@ifstar{\gamma_{k+1}}{\gamma_k}}%
	\newcommand{\Hk}{\@ifstar{H_{k+1}}{H_k}}%
	\newcommand{\rhok}{\@ifstar{\rho_{k+1}}{\rho_k}}%
	\newcommand{\pik}{\@ifstar{\rp_{k+1}}{\rp_k}}%
	\newcommand{\nuk}{\@ifstar{\nu_{k+1}}{\nu_k}}%
	\newcommand{\rk}{\@ifstar{r_{k+1}}{r_k}}%
	\newcommand{\xik}{\@ifstar{\xi_{k+1}}{\xi_k}}%

	\newcommand{\pimin}{\rp_{\rm min}}
	\newcommand{\pimax}{\rp_{\rm max}}
	\newcommand{\rmin}{r_{\rm min}}
	\newcommand{\rmax}{r_{\rm max}}
	\newcommand{\ximin}{\xi_{\rm min}}


	\newcommand{\one}{\mathbbm{1}}

	\newcommand{\changerho}{%
		\renewcommand{\rho}{\varrho}%
		\makeatletter\def\rhot{\@ifstar{\rho_{t+1}}{\rho_t}}\makeatother
	}%



%% Tikz and pgfplots ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

	\pgfplotsset{compat=1.18}
	\pgfplotsset{
		myaxis/.style = {
			grid = major,
			grid style = {dashed, line width = .1pt, draw = gray!10},
			major grid style = {line width = .2pt, draw = gray!50},
			legend style = {at = {(0.5,1.25)}, anchor = south, legend columns = -1, font = {\algnamefont}},
		},
		myaxisD/.style = {
			myaxis,
			xlabel = {\# of calls to \(\linop\) and \(\linop*\)},
		},
		leftto/.style = {
			at = (#1.south east),
			xshift = 2.3cm,
			ylabel = {},
		},
		top/.style = {%
			xlabel = {},
		},
		PGaxis/.style = {
			myaxis,
			xmin = 0,
			ylabel = {$\varphi(x^k) - \min\varphi$},
		},
		gamaxis/.style = {
			myaxis,
			xlabel = {\# of iterations},
			ylabel = {$\gamma_k$},
			legend style = {at = {(0.5,1.05)},legend columns = 3},%
		},
	}

	\pgfplotsset{
		plotline/.style 2 args = {
			very thick,
			mark = {#1},
			color = {#2},
			mark size = 3pt,
			mark options = {solid},
			mark repeat = 5,
			mark phase = 1,
		},
		plotline*/.style 2 args = {
			plotline = {#1}{#2},
			dashed,
		},
		PG-ls11/.style = {%
			plotline* = {square}{teal},
		},
		PG-ls15/.style = {%
			plotline* = {x}{teal},
		},
		PG-ls2/.style = {%
			plotline* = {o}{teal},
		},
		PG-ls13/.style = {%
			plotline* = {diamond}{teal},
		},
		Nesterov/.style = {
			plotline = {x}{red},
		},
		% aGraal/.style = {
		% 	plotline* = {o}{violet},
		% },
		MM/.style = {
			plotline = {square}{blue},
			mark size = 2.7pt,
			mark options = {dashed},
		},
		oursPG/.style = {%
			plotline = {triangle}{black},
		},
		oursPG1/.style = {%
			plotline = {triangle}{green},
			solid,
			% mark size = 2.7pt,
			% mark options = {dashed},
		},
		oursPG2/.style = {%
			plotline = {triangle}{violet},
			dashed,
			% mark options = {dashed},mark size = 2.7pt,
		},
		oursPG3/.style = {%
			plotline = {triangle}{cyan},
			dashed
			% mark options = {dashed},mark size = 2.7pt,
		},
		oursPG4/.style = {%
			plotline = {triangle}{brown},
			solid
			% mark options = {dashed},mark size = 2.7pt,
		},
		oursPGlb/.style = {%
			plotline = {triangle}{orange},
			solid,
			% mark options = {dashed},mark size = 2.7pt,
		},
		% oursPD/.style = {%
		% 	oursPG,
		% },
		% oursPD+/.style = {%
		% 	plotline* = {square}{black},
		% },
	}


% Revision and comments ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

% 	\newcommand{\missing}{{\Red MISSING}}
% 	\newcommand{\note}[1]{{\red\sffamily(#1)}}
% 	\pretocmd\grayout{\ifshowgray\else{\gray\hrule\hspace*{0pt}\hfill (removed content)\hfill\hspace*{0pt}\hrule}}{}{}
	\colorlet{grayoutcolor}{gray!35}
\makeatother


==> TeX/Text/Simulations/PG/cubic.tex <==
The subproblem in the cubic Newton method \cite{nesterov2006cubic} involves solving
\[
    \minimize_{x\in \R^{n+1}} \; \tfrac12\innprod{x}{Qx} + \innprod{x}{q} + \tfrac{M}{6}\|x\|^3,
\]
where \(Q\in\R^{(n+1)\times (n+1)}\), \(q\in\R^{n+1}\), and \(M>0\) is some regularization parameter.
In the simulations, the Hessian \(Q\) and the gradient \(q\) are generated for the logistic loss problem evaluated at zero on the mushroom, a5a, and phishing datasets.
Moreover, \(M= 1\) is used in the plots, though we remark that the behavior of the algorithms for different values is similar.


==> TeX/Text/Simulations/PG/lasso.tex <==
Consider the lasso problem
\[
	\minimize_{x\in\R^n}\tfrac12\|Dx - b\|^2 + \|x\|_1,
\]
where matrix \(D\in \R^{m\times n}\) and vector \(b\in \R^n\) are generated based on the procedure described in \cite[\S6]{nesterov2013gradient}, and \(n_\star\) denotes the number of nonzero elements of the solution.
In all simulations, the parameter controlling the magnitude of the primal solution was set equal to one (\(\rho = 1\) in the notation of \cite[\S6]{nesterov2013gradient}), but the general behavior of the algorithms is similar for alternative values.


==> TeX/Text/Simulations/PG/logreg.tex <==
We consider an \(\ell_1\)-regularized logistic regression problem
\[
	\minimize_{x\in \R^{n+1}} \; -\tfrac1m
	\textstyle
	\sum_{i=1}^m
	\Bigl[
		y_i \log\bigl(s_i(x)\bigr)
		+
		(1-y_i)\log\bigl(1-s_i(x)\bigr)
	\Bigr]
	+ \lambda \|x\|_1,
\]
where \(\lambda>0\) is the regularization parameter, \(m,n\) are the number of samples and features,
\(
	s_i(x)
=
	(1+ \exp(-\trans{d_i}x))^{-1}
\)
are logistic sigmoid functions with \(d_i\in\R^{n+1}\) denoting the \(i\)-th data sample (up to absorbing the bias terms), and \(y_i\in\set{0,1}\) is the associated label.
In \cref{fig:logreg} the algorithms are compared in terms of the total number of calls to \(D\) and its adjoint, where \(D\) denotes the data matrix constructed by stacking the vectors \(d_i\).
In all the simulations \(\lambda = 0.01\) was used.


==> TeX/Tikz/cubic_logreg.tex <==
%!TEX root = ../../adaAMA.tex
\begin{tikzpicture}
	\begin{axis}[
		PGaxis,
		ymode = log,
		name = m1,
		xmax = 5e1,
		xlabel = {\# of calls to linear operators},
		title = {a5a dataset  (\(m = 6414, n = 123\), density\({}=0.11\))},
	]
		% \addplot[Nesterov]
			% file {TeX/Tikz/plot_data/cubic_logreg/Nesterov(fixed)-a5a.jsonl.txt};

		\addplot[PG-ls13]
			file {TeX/Tikz/plot_data/cubic_logreg/PGM(backtracking)-(xi=1.3)-a5a.jsonl.txt};

		\addplot[MM]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(MM)-a5a.jsonl.txt};

		\addplot[oursPG]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(ours)-a5a.jsonl.txt};

		\addplot[oursPG1]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.67,1,0.83)-a5a.jsonl.txt};

		\addplot[oursPG2]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.11,1,0.83)-a5a.jsonl.txt};

		\addplot[oursPG4]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.5,1,0.75)-a5a.jsonl.txt};

		\addplot[oursPG3]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(2.5,1,1.0)-a5a.jsonl.txt};


		\addplot[oursPGlb]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.0,1,0.5)-a5a.jsonl.txt};

	\end{axis}
	\begin{axis}[
		PGaxis,
		leftto = {m1},
		ymode = log,
		name = m2,
		xmax = 5e1,
		xlabel = {\# of calls to linear operators},
		title  = {mushroom dataset (\(m = 8124, n = 112\), density\({}=0.19\))},
	]
		% \addplot[Nesterov]
			% file {TeX/Tikz/plot_data/cubic_logreg/Nesterov(fixed)-mushrooms.jsonl.txt};

		\addplot[PG-ls11]
			file {TeX/Tikz/plot_data/cubic_logreg/PGM(backtracking)-(xi=1.1)-mushrooms.jsonl.txt};

		\addplot[MM]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(MM)-mushrooms.jsonl.txt};

		\addplot[oursPG]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(ours)-mushrooms.jsonl.txt};

		\addplot[oursPG1]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.67,1,0.83)-mushrooms.jsonl.txt};

		\addplot[oursPG2]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.11,1,0.83)-mushrooms.jsonl.txt};


		\addplot[oursPG4]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.5,1,0.75)-mushrooms.jsonl.txt};

		\addplot[oursPG3]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(2.5,1,1.0)-mushrooms.jsonl.txt};

		\addplot[oursPGlb]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.0,1,0.5)-mushrooms.jsonl.txt};
	\end{axis}
	\begin{axis}[
		PGaxis,
		leftto = {m2},
		ymode = log,
		name = m3,
		xmax = 30,
		xlabel = {\# of calls to linear operators},
		title = {phishing dataset  (\(m = 11055, n = 68\), density\({}=0.44\))},
	]
		% \addplot[Nesterov]
			% file {TeX/Tikz/plot_data/cubic_logreg/Nesterov(fixed)-phishing.jsonl.txt};

		\addplot[PG-ls15]
			file {TeX/Tikz/plot_data/cubic_logreg/PGM(backtracking)-(xi=1.5)-phishing.jsonl.txt};

		\addplot[MM]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(MM)-phishing.jsonl.txt};

		\addplot[oursPG]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(ours)-phishing.jsonl.txt};

		\addplot[oursPG1]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.67,1,0.83)-phishing.jsonl.txt};

		\addplot[oursPG2]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.11,1,0.83)-phishing.jsonl.txt};

		\addplot[oursPG4]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.5,1,0.75)-phishing.jsonl.txt};

		\addplot[oursPG3]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(2.5,1,1.0)-phishing.jsonl.txt};


		\addplot[oursPGlb]
			file {TeX/Tikz/plot_data/cubic_logreg/AdaPGM(p,nu,r)(1.0,1,0.5)-phishing.jsonl.txt};
	\end{axis}
\end{tikzpicture}



==> TeX/Tikz/gammaPD.tex <==
\begin{tikzpicture}[scale = 0.5]
	\begin{axis}[
		gamaxis, ymode = log,
		name = m3,
		xlabel = {\# of{}  calls to \(\nabla f\)},
		xmin = 50,
		xmax = 100,
	]

		\addplot[MP]
			file {TeX/Tikz/plot_data/dsvm_C01/gam/MP_8124_112_10_1000.txt};

		\addplot[oursPD]
			file {TeX/Tikz/plot_data/dsvm_C01/gam/APDHG_8124_112_10_1000.txt};

		\legend{MP-ls, \adaPD, \adaPD+}
	\end{axis}
	\begin{axis}[
		gamaxis, ymode = log,
		leftto = m3,
		xlabel = {\# of{}  calls to \(\linop\) and \(\linop*\)},
		xmin = 50,
		xmax = 100,
	]
		\addplot[MP, each nth point={1}]
			file {TeX/Tikz/plot_data/medreg1_ell1/gam/MP_506_13_1000_1000.txt};

		\addplot[oursPD+, each nth point={1}]
			file {TeX/Tikz/plot_data/medreg1_ell1/gam/adaPD+_506_13_1000_1000.txt};

		\legend{MP-ls, \adaPD+}
	\end{axis}
\end{tikzpicture}



==> TeX/Tikz/gammaPG.tex <==
\begin{tikzpicture}[scale = 0.5]
	\begin{axis}[
		gamaxis, ymode = log,
		name = m1,
		xlabel = {\# of calls to \(D\) and \(\trans D\)},
		xmin = 50,
		xmax = 150,
		restrict x to domain = 50:150,
	]
		\addplot[aGraal]
			file {TeX/Tikz/plot_data/logreg/gam/aGraal_8124_113_1_1.txt};

		\addplot[Nesterov]
			file {TeX/Tikz/plot_data/logreg/gam/Nesterov_bt_8124_113_1_1.txt};

		\addplot[PG-ls]
			file {TeX/Tikz/plot_data/logreg/gam/PGM_bt-1.5_8124_113_1_1.txt};

		\addplot[PG]
			file {TeX/Tikz/plot_data/logreg/gam/PGM_fixed_8124_113_1_1.txt};

		\addplot[MM]
			file {TeX/Tikz/plot_data/logreg/gam/PGM_MM_8124_113_1_1.txt};

		\addplot[oursPG]
			file {TeX/Tikz/plot_data/logreg/gam/PGM_our_8124_113_1_1.txt};

		\legend{aGRAAL, Nesterov, PGM-ls, PGM, \adaPG-MM, \adaPG}

	\end{axis}
	\begin{axis}[
		gamaxis, ymode = log,
		leftto = m1,
		name = m2,
		xlabel = {\# of calls to \(D\) and \(\trans D\)},
		xmin = 50,
		xmax = 150,
		restrict x to domain = 50:150,
	]

	    \addplot[aGraal]
        file {TeX/Tikz/plot_data/lasso/gam/aGRAAL-lasso_500_1000_10.jsonl.txt};

    \addplot[Nesterov]
        file {TeX/Tikz/plot_data/lasso/gam/Nesterov(backtracking)-lasso_500_1000_10.jsonl.txt};

    \addplot[PG-ls2]
        file {TeX/Tikz/plot_data/lasso/gam/PGM(backtracking)-(xi=1.5)-lasso_500_1000_10.jsonl.txt};

    \addplot[PG]
        file {TeX/Tikz/plot_data/lasso/gam/PGM(fixed)-lasso_500_1000_10.jsonl.txt};

    \addplot[MM]
        file {TeX/Tikz/plot_data/lasso/gam/AdaPGM(MM)-lasso_500_1000_10.jsonl.txt};

    \addplot[oursPG]
        file {TeX/Tikz/plot_data/lasso/gam/AdaPGM(ours)-lasso_500_1000_10.jsonl.txt};

	\legend{aGRAAL, Nesterov, PGM-ls, PGM, \adaPG-MM, \adaPG}
	\end{axis}
\end{tikzpicture}



==> TeX/Tikz/lasso.tex <==
%!TEX root = ../../adaAMA.tex
\begin{tikzpicture}
	\begin{axis}[
		PGaxis,
		ymode = log,
		name = m1,
		xmax = 2e3,
		% xlabel = {\# of calls to \(D\) and \(\trans D\)},
		xlabel = {\hphantom{a5a dataset (\(m = 6414, n = 123\), density\({}=0.11\))}},
		title = {$m = 100$, $n=300$, $n_\star=30$},
	]

		\addplot[Nesterov, name=Nesterov]
			file {TeX/Tikz/plot_data/lasso/Nesterov(fixed)-lasso_100_300_10.jsonl.txt};


		\addplot[MM, name=MM]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(MM)-lasso_100_300_10.jsonl.txt};

		\addplot[oursPG, name=adaPG]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(ours)-lasso_100_300_10.jsonl.txt};

		\addplot[oursPG1, name=adaPG1]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.67,1,0.83)-lasso_100_300_10.jsonl.txt};

		\addplot[oursPG2, name=adaPG2]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.11,1,0.83)-lasso_100_300_10.jsonl.txt};

		\addplot[oursPG4, name=adaPG4]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.5,1,0.75)-lasso_100_300_10.jsonl.txt};

		\addplot[oursPG3, name=adaPG3]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(2.5,1,1.0)-lasso_100_300_10.jsonl.txt};


		\addplot[oursPGlb, name=adaPGlb]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.0,1,0.5)-lasso_100_300_10.jsonl.txt};

		\addplot[PG-ls15, name=ls]
			file {TeX/Tikz/plot_data/lasso/PGM(backtracking)(xi=1.5)-lasso_100_300_10.jsonl.txt};


	\end{axis}
	\begin{axis}[
		PGaxis,
		leftto = {m1},
		ymode = log,
		name = m2,
		xmax = 2.5e3,
		% xlabel = {\# of calls to \(D\) and \(\trans D\)},
		xlabel = {\hphantom{mushroom dataset (\(m = 8124, n = 112\), density\({}=0.19\))}},
		title = {$m = 500$, $n=1000$, $n_\star=100$},
	]

		\addplot[Nesterov, name=Nesterov]
			file {TeX/Tikz/plot_data/lasso/Nesterov(fixed)-lasso_500_1000_10.jsonl.txt};


		\addplot[MM, name=adaPG-MM]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(MM)-lasso_500_1000_10.jsonl.txt};

		\addplot[oursPG, name=adaPG]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(ours)-lasso_500_1000_10.jsonl.txt};

		\addplot[oursPG1, name=adaPG1]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.67,1,0.83)-lasso_500_1000_10.jsonl.txt};

		\addplot[oursPG2, name=adaPG2]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.11,1,0.83)-lasso_500_1000_10.jsonl.txt};

		\addplot[oursPG4, name=adaPG4]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.5,1,0.75)-lasso_500_1000_10.jsonl.txt};

		\addplot[oursPG3, name=adaPG3]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(2.5,1,1.0)-lasso_500_1000_10.jsonl.txt};


		\addplot[oursPGlb, name=adaPGlb]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.0,1,0.5)-lasso_500_1000_10.jsonl.txt};


		\addplot[PG-ls13, name=PGM-ls]
			file {TeX/Tikz/plot_data/lasso/PGM(backtracking)(xi=1.3)-lasso_500_1000_10.jsonl.txt};
		\legend{
		Nesterov,
		adaPG-MM,
		adaPG,
		adaPG\(^{(\frac53,\frac56)}\),
		adaPG\(^{(\frac{10}{9}, \frac56)}\),
		adaPG\(^{(\frac{3}{2}, \frac34)}\),
		adaPG\(^{(\frac{5}{2}, 1)}\),
		adaPG\(^{(1, \frac12)}\)
		}
	\end{axis}
	\begin{axis}[%
    hide axis,
    xmin=10,
    xmax=50,
    ymin=0,
    ymax=0.4,
    legend style = {at = {(1.83,1.13)}, draw=white!15!black, anchor = south, legend columns = -1, font = {\algnamefont}},
    ]

	\addlegendimage{teal,mark=square, dash pattern=on 3pt off 1pt on 3pt off 1pt, mark options={scale=1.2,thick, solid}, line width=1.5pt}
    \addlegendentry{PG-ls\(^{1.1}\)};

    \addlegendimage{teal,mark=diamond, dash pattern=on 3pt off 1pt on 3pt off 1pt, mark options={scale=1.3,thick, solid}, line width=1.5pt}
    \addlegendentry{PG-ls\(^{1.3}\)};


	\addlegendimage{teal,mark = x, dash pattern=on 3pt off 1pt on 3pt off 1pt, mark options={scale=1.3,thick, solid}, line width=1.5pt}
    \addlegendentry{PG-ls\(^{1.5}\)};


	\addlegendimage{teal,mark=o, dash pattern=on 3pt off 1pt on 3pt off 1pt, mark options={scale=1.3,thick, solid}, line width=1.5pt}
    \addlegendentry{PG-ls\(^{2}\)};
    \end{axis}
	\begin{axis}[
		PGaxis,
		leftto = {m2},
		ymode = log,
		name = m3,
		xmax = 1e3,
		% xlabel = {\# of calls to \(D\) and \(\trans D\)},
		xlabel = {\hphantom{phishing dataset (\(m = 11055, n = 68\), density\({}=0.44\))}},
		title = {$m = 4000$, $n=1000$, $n_\star=100$},
	]

		\addplot[Nesterov]
			file {TeX/Tikz/plot_data/lasso/Nesterov(fixed)-lasso_4000_1000_10.jsonl.txt};

		\addplot[MM]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(MM)-lasso_4000_1000_10.jsonl.txt};

		\addplot[oursPG]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(ours)-lasso_4000_1000_10.jsonl.txt};

		\addplot[oursPG1]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.67,1,0.83)-lasso_4000_1000_10.jsonl.txt};

		\addplot[oursPG2]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.11,1,0.83)-lasso_4000_1000_10.jsonl.txt};


		\addplot[oursPG4]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.5,1,0.75)-lasso_4000_1000_10.jsonl.txt};

		\addplot[oursPG3]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(2.5,1,1.0)-lasso_4000_1000_10.jsonl.txt};

		\addplot[oursPGlb]
			file {TeX/Tikz/plot_data/lasso/AdaPGM(p,nu,r)(1.0,1,0.5)-lasso_4000_1000_10.jsonl.txt};

		\addplot[PG-ls2]
			file {TeX/Tikz/plot_data/lasso/PGM(backtracking)(xi=2.0)-lasso_4000_1000_10.jsonl.txt};
	\end{axis}
\end{tikzpicture}


==> TeX/Tikz/logreg.tex <==
%!TEX root = ../../adaAMA.tex
\begin{tikzpicture}
	\begin{axis}[
		PGaxis,
		ymode = log,
		name = m1,
		xmax = 700,
		% xlabel = {\# of calls to \(D\) and \(\trans D\)},
		title = {a5a dataset (\(m = 6414, n = 123\), density\({}=0.11\))},
	]

		\addplot[Nesterov]
			file {TeX/Tikz/plot_data/logreg/Nesterov(fixed)-a5a.jsonl.txt};

		\addplot[PG-ls15]
			file {TeX/Tikz/plot_data/logreg/PGM(backtracking)-(xi=1.5)-a5a.jsonl.txt};

		\addplot[MM]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(MM)-a5a.jsonl.txt};

		\addplot[oursPG]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(ours)-a5a.jsonl.txt};

		\addplot[oursPG1]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.67,1,0.83)-a5a.jsonl.txt};

		\addplot[oursPG2]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.11,1,0.83)-a5a.jsonl.txt};


		\addplot[oursPG4]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.5,1,0.75)-a5a.jsonl.txt};

		\addplot[oursPG3]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(2.5,1,1.0)-a5a.jsonl.txt};


		\addplot[oursPGlb]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.0,1,0.5)-a5a.jsonl.txt};


	\end{axis}
	\begin{axis}[
		PGaxis,
		leftto = {m1},
		ymode = log,
		name = m2,
		xmax = 2e3,
		% xlabel = {\# of calls to \(D\) and \(\trans D\)},
		title  = {mushroom dataset (\(m = 8124, n = 112\), density\({}=0.19\))},
	]

		\addplot[Nesterov]
			file {TeX/Tikz/plot_data/logreg/Nesterov(fixed)-mushrooms.jsonl.txt};

		\addplot[PG-ls2]
			file {TeX/Tikz/plot_data/logreg/PGM(backtracking)-(xi=2.0)-mushrooms.jsonl.txt};

		\addplot[MM]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(MM)-mushrooms.jsonl.txt};

		\addplot[oursPG]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(ours)-mushrooms.jsonl.txt};

		\addplot[oursPG1]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.67,1,0.83)-mushrooms.jsonl.txt};

		\addplot[oursPG2]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.11,1,0.83)-mushrooms.jsonl.txt};

		\addplot[oursPG4]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.5,1,0.75)-phishing.jsonl.txt};
		\addplot[oursPG3]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(2.5,1,1.0)-mushrooms.jsonl.txt};


		\addplot[oursPGlb]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.0,1,0.5)-mushrooms.jsonl.txt};

	\end{axis}
	\begin{axis}[
		PGaxis,
		leftto = {m2},
		ymode = log,
		name = m3,
		xmax = 2e3,
		% xlabel = {\# of calls to \(D\) and \(\trans D\)},
		title = {phishing dataset (\(m = 11055, n = 68\), density\({}=0.44\))},
	]

		\addplot[Nesterov]
			file {TeX/Tikz/plot_data/logreg/Nesterov(fixed)-phishing.jsonl.txt};

		\addplot[PG-ls15]
			file {TeX/Tikz/plot_data/logreg/PGM(backtracking)-(xi=1.5)-phishing.jsonl.txt};

		\addplot[MM]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(MM)-phishing.jsonl.txt};

		\addplot[oursPG]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(ours)-phishing.jsonl.txt};

		\addplot[oursPG1]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.67,1,0.83)-phishing.jsonl.txt};

		\addplot[oursPG2]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.11,1,0.83)-phishing.jsonl.txt};

		\addplot[oursPG4]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.5,1,0.75)-phishing.jsonl.txt};

		\addplot[oursPG3]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(2.5,1,1.0)-phishing.jsonl.txt};

		\addplot[oursPGlb]
			file {TeX/Tikz/plot_data/logreg/AdaPGM(p,nu,r)(1.0,1,0.5)-phishing.jsonl.txt};
	\end{axis}
\end{tikzpicture}


